Integer Reasoning Modulo Different Constants in SMT

This paper presents a new refutation procedure for multimodular systems of integer constraints that commonly arise when verifying cryptographic protocols. These systems, involving polynomial equalities and disequalities modulo different constants, are challenging for existing solvers due to their inability to exploit multimodular structure. To address this issue, our method partitions constraints by modulus and uses lifting and lowering techniques to share information across subsystems, supported by algebraic tools like weighted Gr\"obner bases. Our experiments show that the proposed method outperforms existing state-of-the-art solvers in verifying cryptographic implementations related to Montgomery arithmetic and zero-knowledge proofs.

==> float/calculus/liftEqH.tex <==
\begin{figure}[t]
\begin{center}
\def\defaultHypSeparation{\hskip .01in}
 \AxiomC{$p \in \WeightedGB(\REqsN)$}
 \AxiomC{ $q \in \{p, \inv(p)\}$} {\hskip 0.5em}
 \AxiomC{$\liftN(q,B)$} {\hskip 0.5em}
 \AxiomC{$ q  \notin I_{\Int}(\IntEqs) $}
 \LeftLabel{\HeuristicGB}
 \alwaysSingleLine
 \QuaternaryInfC{$\IntEqs := \IntEqs, q$ }
 \DisplayProof
 \end{center}
\caption{Refined rule for lifting based on \WeightedGB, replacing \LiftEq.}
\label{fig:liftEqH}
\end{figure}

==> float/calculus/optimizations.tex <==
\begin{figure}[t]
 \begin{center}
 \def\defaultHypSeparation{\hskip .01in}
  \AxiomC{$ \dbk{e} \in I_{n}(\dbk{\REqsN})$}
  \AxiomC{$n \neq \infty$}
  \alwaysNoLine
  \def\extraVskip{2pt}
  \BinaryInfC{$\CalcBds(B,e) \not\subseteq [1-n,n-1]$ {\hskip .03in} $\CalcBds(B,e) \subseteq [1-2n, 2n-1]$ }
  \def\extraVskip{2pt}
  \UnaryInfC{ $ \dbk{e-n} \notin I_{\infty}(\dbk{\IntEqs})$ {\hskip .03in} $ \dbk{e} \notin I_{\infty}(\dbk{\IntEqs}) $ {\hskip .03in} $ \dbk{e+n} \notin I_{\infty}(\dbk{\IntEqs})$}
  % \def\extraVskip{2pt}
  % \alwaysNoLine
  %  \UnaryInfC{$\CalcBds(B,e) \not\subseteq [1-n,n-1]$ {\hskip .03in} $\CalcBds(B,e) \subseteq [2-2n, 2n-2]$ }
\LeftLabel{\RngLift}
\alwaysSingleLine
\UnaryInfC{$\IntEqs := \IntEqs, e - n \branch \IntEqs := \IntEqs, e \branch \IntEqs := \IntEqs, e+n$}
  \DisplayProof
\end{center}
\begin{center}
\def\defaultHypSeparation{\hskip .01in}
  \AxiomC{$ \dbk{e}  \in I_{n}(\dbk{\REqsN})$}
  \AxiomC{$ e = s^2 -s$}
   \alwaysNoLine
  \def\extraVskip{2pt}
  \BinaryInfC{ $n \neq \infty$ {\hskip .03in} \texttt{IsPrime}($n$)  {\hskip .03in} $ \dbk{s} \notin I_{n}(\dbk{\REqsN})$ {\hskip .03in} $\dbk{s-1} \notin I_{n}(\dbk{\REqsN}) $ }
  \LeftLabel{\PrimeSqr}
  \alwaysSingleLine
  \UnaryInfC{ $\REqsN := \REqsN, s \branch \REqsN := \REqsN, s-1$}
  \DisplayProof
\end{center}
\caption{Branching rules: $e$ and $s$ are expressions.}
\label{fig:opt_rules}
\end{figure}



==> float/calculus/preprocess.tex <==
\begin{figure}[ht]
% \begin{center}
%     \AxiomC{$s \SMTdiv c = t$}
% \LeftLabel{DivEq}
% \UnaryInfC{X:= R, Q \quad L := $R \geq 0 , R \leq c, (s-R) \bmod c = 0, s-R =c*q$ }
%   \DisplayProof
% \end{center}
% \begin{center}
% \def\defaultHypSeparation{\hskip .0001in}
%     \AxiomC{$ s \geq t$ }
%     \LeftLabel{ExpGEQ}
%     \UnaryInfC{X:=$X_j$ \quad L:= ($s-t = X_j$) \quad B[$X_j$][0]:= 0 }
%     \DisplayProof
% \end{center}
% \begin{center}
% \def\defaultHypSeparation{\hskip .0001in}
%     \AxiomC{$ s \leq t$ }
%     \LeftLabel{ExpLEQ}
%     \UnaryInfC{X:=$X_j$ \quad L:= ($s-t = X_j$) \quad B[$X_j$][1]:= 0 }
%     \DisplayProof
  % \end{center}

 \begin{center}
\AxiomC{ $\bowtie \ \in \{ \approx, \not \approx \}$}
  \AxiomC{$(s \bmod n \bowtie 0) \in L$}
\LeftLabel{\ModExp}
\BinaryInfC{$L:= L \setminus \{ s \bmod n \bowtie 0\} \quad \RMod^{\bowtie} := \RMod^{\bowtie}, \dbk{\toPoly(s)}_n$}
  \DisplayProof
\end{center}
% \begin{center}
%  \AxiomC{$s \bmod c \neq 0$}
% \LeftLabel{ModDiseq}
% \UnaryInfC{\RNEqs := \RNEqs, $\dbk{\toPoly(s)}_c$}
%   \DisplayProof
% \end{center}
\begin{center}
\AxiomC{ $\bowtie \ \in \{ \approx, \not \approx \}$}
 \AxiomC{$ (s \bowtie  0) \in L$}
\LeftLabel{\IntExp}
\BinaryInfC{ $L:= L\setminus \{s \bowtie 0\} \quad R_{\Int}^{\bowtie} := R_{\Int}^{\bowtie} , \toPoly(s)$}
  \DisplayProof
\end{center}
% \begin{center}
% \AxiomC{$s \neq t$}
% \LeftLabel{IntDiseq}
% \UnaryInfC{\IntNEqs := \IntNEqs, $\toPoly(s-t)$}
%   \DisplayProof
% \end{center}
\begin{center}
\AxiomC{$(x\geq n) \in L$}
\LeftLabel{\GEQ}
\UnaryInfC{$L:= L\setminus \{x \geq n\} \quad B(x)_1$ := $\max(B(x)_1, n)$}
  \DisplayProof
\end{center}

\begin{center}
\def\defaultHypSeparation{\hskip .01in}
\AxiomC{$(x \leq n) \in L$ }
\LeftLabel{\LEQ}
\UnaryInfC{$L:= L\setminus \{x \leq c\} \quad B(x)_2$ := $\min(B(x)_2, n) $}
  \DisplayProof
\end{center}

\begin{center}
\AxiomC{$\neg(x\geq n) \in L$}
\LeftLabel{\nGEQ}
\UnaryInfC{$L:= L\setminus \{\neg(x \geq n)\} \quad B(x)_2 := \min(B(x)_2, n+1)$}
  \DisplayProof
\end{center}

\begin{center}
\AxiomC{$\neg(x\leq n) \in L$}
\LeftLabel{\nLEQ}
\UnaryInfC{$L:= L\setminus \{\neg(x \leq n)\ \quad B(x)_1:= \max(B(x)_1, n-1)$}
  \DisplayProof
\end{center}



\caption{Algebraic encoding rules}
\label{fig:preprocess_rules}
\end{figure}

